QPoser: Quantized Explicit Pose Prior Modeling for Controllable Pose Generation

Explicit pose prior models compress human poses into latent representations for using in pose-related downstream tasks. A desirable explicit pose prior model should satisfy three desirable abilities: 1) correctness, i.e. ensuring to generate physically possible poses; 2) expressiveness, i.e. ensuring to preserve details in generation; 3) controllability, meaning that generation from reference poses and explicit instructions should be convenient. Existing explicit pose prior models fail to achieve all of three properties, in special controllability. To break this situation, we propose QPoser, a highly controllable explicit pose prior model which guarantees correctness and expressiveness. In QPoser, a multi-head vector quantized autoencoder (MS-VQVAE) is proposed for obtaining expressive and distributed pose representations. Furthermore, a global-local feature integration mechanism (GLIF-AE) is utilized to disentangle the latent representation and integrate full-body information into local-joint features. Experimental results show that QPoser significantly outperforms state-of-the-art approaches in representing expressive and correct poses, meanwhile is easily to be used for detailed conditional generation from reference poses and prompting instructions.

==> figs/cover_tradeoff.tex <==
% Use figure* for multi-column figure
\begin{figure}[tp]
    \centering
    \begin{subfigure}[t]{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs/cover/area cover small.pdf}
        \caption{Correct but not expressive, include too little}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figs/cover/cover all.pdf}
         \caption{Expressive but not correct, include too much}
    \end{subfigure}
    \caption{It is difficult to learn the complex manifold border, and current pose priors often have to trade between expressiveness(include all plausible poses) and correctness(exclude implausible poses).}
    \label{fig:cover_tradeoff}
\end{figure}


==> figs/smoothness.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/smoothness/smoothness.png}
    \caption{\textbf{Comparison:}
    We compare the smoothness by evaluating how much(percentage) joints rotate at each step in latent interpolation. Note that the value doesn't necessarily add up to 100\%, as the total is the MPJAE between the initial and destination pose. We show that our model is comparable with existing models in smoothness, with smooth and stable adjustments between steps. We also show the qualitative results in \ref{fig:comparison}.
    }
    \label{fig:smoothness}
\end{figure}

